An authentication protocol based on chaos and zero knowledge proof

Port Knocking is a method for authenticating clients through a closed stance firewall, and authorising their requested actions, enabling severs to offer services to authenticated clients, without opening ports on the firewall. Advances in port knocking have resulted in an increase in complexity in design, preventing port knocking solutions from realising their potential. This paper proposes a novel port knocking solution, named Crucible, which is a secure method of authentication, with high usability and features of stealth, allowing servers and services to remain hidden and protected. Crucible is a stateless solution, only requiring the client memorise a command, the server's IP and a chosen password. The solution is forwarded as a method for protecting servers against attacks ranging from port scans, to zero-day exploitation. To act as a random oracle for both client and server, cryptographic hashes were generated through chaotic systems.

==> 06_con.tex <==

\section{Conclusions}
Port knocking was discussed in the introductory chapter as an authentication mechanism with an `image problem'. In this dissertation, extensive coverage of literature on port knocking, and on cryptographic topics, has directed practical experiments towards finding a port knocking solution that hopefully serves to improve this image. \\

% three prototypes

The experimental process of prototyping used in the dissertation, a series of mutations and improvements on the original design, has produced a hardened protocol. Crucible is a secure method of authentication, with high usability, and features of stealth, the latter allowing servers and services to remain hidden {\it and} protected from adversaries. Crucible would not require drastic changes to adapt itself for different platforms, and in doing so, could be used to defend from the most innocent port scan, to a zero-day attack, on devices ranging from small embedded platforms in home appliances, to workhorse servers in an enterprise setting.\\

Throughout the process in designing a secure prototype, manifestations of larger themes in security have been seen. The security versus obscurity debate has raised questions over the extent to which features such as stealth should be prioritised, but also has highlighted that obscurity can {\it complement} security in reducing certain attacks. The axiom ``complexity is the worst enemy of security'' \parencite{1ah} has resulted in a port knocking solution that has had to forgo shiny features in place of grounded security foundations, indeed many of the design `decisions' were already made in keeping with reducing complexity. Even some of the most simple operations, such as adding a nonce before hashing, has proved to have large underlying security implications and considerations.\\

% proving itself in the field of battle
% series of mutating prototypes -- creation and destruction

The following section analyses whether the objectives set out at the beginning of the dissertation have been met. Future work is then offered, divided into lower-level improvements on Crucible as a development project, and more general research tasks, for both Crucible and further research in port knocking. Lastly, the author's personal reflections of the dissertation are recounted.
\pagebreak

\section{Achievement of Objectives}
{\bf Objective \ref{obj:I}: }Develop a secure port knocking prototype that improves on the drawbacks of existing solutions and demonstrates the ability to securely authenticate clients and authorise commands.
\begin{itemize}
    \item[] The experimental trial-and-error process has produced a Crucible, a port knocking solution resistant to the weaknesses of its predecessors. Crucible was then subjected to a number of theoretical attacks in an open and transparent evaluation aimed at finding the protocol's flaws. Crucible's security has been appraised to the best of the author's ability and found to have no largely concerning weaknesses. Beyond the scope of this dissertation, Crucible's security would be more effectively appraised through formal cryptographic audit. Better assurance could be provided by a cryptographic proof of security.
\end{itemize}

{\bf Objective \ref{obj:II}: }Examine literature and port knocking implementations to classify the design and mechanical features of port knocking solutions in a manner that benefits the design process for future developers.
\begin{itemize}
    \item[] The literature review in the second chapter examined a large body of work and, as a novel approach, decomposed the work into a classification of port knocking features categorised by mechanics and architecture. In doing so, the author aimed to allow future developers to selectively implement or exclude modular components of existing port knocking implementations, based on their merit. As a result, the work should hopefully form a beneficial reference for future development projects.
\end{itemize}

{\bf Objective \ref{obj:III}: }Introduce the reader to areas of theoretical cryptography, in a manner that is easily understood, and applicable to other security projects.
\begin{itemize}
    \item[] The third chapter on design and methodology introduced the reader to random beacons, zero knowledge proofs and chaos-based cryptography. Particularly for the latter topics, a large amount of the literature referred to was challenging to approach. In this dissertation, they are presented with pedagogical parables, metaphor and examples, in the aim to make them clearly understood. From these topics, functional protocols and algorithms were found, and implemented during experimentation. Hopefully their qualities as laid out in the text will inform decision for their use in other security projects.
\end{itemize}

{\bf Objective \ref{obj:IV}: }Leverage theoretical fields of research in creating the port knocking protocol and provide a general case study demonstrating the merits and drawbacks of incorporating largely theoretical cryptography into practical applications.
\begin{itemize}
    \item[] The trial-and-error nature of developing Crucible permuted the Bitcoin random beacon, Schnorr's NIZKP and the absolute value chaos-based hash function amongst each prototype iteration. This was not intentional; each successive prototype aimed to improve on the drawbacks of the previous. As a result, Crucible only draws {\it inspiration} from the topics of zero knowledge proofs, and chaos-based cryptography, but does not actually implement their protocols and algorithms. The difficulties encountered in application of the topics were discussed in Section \ref{sec:foreword}. Crucible {\it itself} is however a testament to the merits of applying theoretical concepts into practical development, which it could not have been produced without.
\end{itemize}

{\bf Objective \ref{obj:V}: }Use the development of a port knocking protocol to illustrate the more general case of how secure protocols are designed an evaluated.
\begin{itemize}
    \item[] Appraisal of this objective is hard to quantify. Intentionally the design goals of the prototypes did not favour credence to features, usability, or performance, instead opting to focus heavily on security. Further, a cryptographic narrative has ran throughout the dissertation. The experimental phase of testing and developing new prototypes resulted in the adoption of Crucible, over the other prototypes, by a Darwinian {\it last one standing} approach, designed to root out less secure solutions. Evaluation continued this sentiment by subjecting Crucible to a number of hypothetical attack scenarios, designed to uncover any weak spots.
\end{itemize}

\section{Future Work}
If the prototype were to be progressed into a distributable application, or for production deployment, the following require consideration.\\
% delineate between something that turns it from a prototype into a working solution, 
% and other areas that should be looked into


{\bf Future Development:}
\begin{itemize}
    \item For ease of development in producing a working proof of concept, Python was chosen as the programming language. \parencite{1y} notes that a lower-level programming language could be used, such as C, that could make deployment easier to hardware devices such as firewalls. Further, this may improve server performance. In contrast, \parencite{6i} views memory unsafe languages as undesirable for a port knocking service. 
    \item Given the access that Crucible provides a client, proper channels of logging are required to keep a history of authorised actions, and potential attacks. This should feature options for reliable remote logging, particularly for deployment in an organisation, to ensure accountability of the protocol, integration with existing security infrastructure (e.g. SIEMs) and regulatory compliance.
    \item The knocking server could optionally pass the knock's source IP into a user command, this would not be difficult to integrate into the setup of a profile, and could provide additional granularity in authorisation e.g. opening a port for a specific IP.
    \item Support for multiple users could be added after tackling the problem of fixed salt values, seen in Section \ref{sec:passwords}. In the same vein, password policy could be enforced through Crucible's setup process, to ensure only safe password choices are made by the user.
    \item Trust in the random beacon service could be improved by polling multiple beacon sources (i.e. blockchain APIs) and cross-validating results. Further, a tool could be developed to host a random beacon service, e.g. through a simple http server for a back end PRNG. This could be deployed by clients on a secure machine, such as a VPS. Lastly, random delays could be added to beacon requests, as a stealth measure, to remove identifiable traffic patters from a listening attacker.
\end{itemize}
\newpage

{\bf Future Research:}\label{sec:future}
\begin{itemize}
    \item The listening service (libpcap via scapy) has already been flagged for its lack of stealth, potential DoS and exploitation vectors and privilege requirements. \parencite{1z} offers discussion on alternatives to sniffers: parsing firewall logs as a medium of retrieving knock data. This was explored briefly (and admittedly, inadequately) and deemed to be a difficult option, without either having to embed authenticating data into the packet options (see Section \ref{sec:medium}), or modify the firewall to support full-payload logging. 
    \item \parencite{1d} features per-knock randomisation of the client source IP address, this has the benefit of making client identification more difficult for an attacker, and could serve as an authentication medium. However, firewall restrictions in a secure subnet should only allow egress from traffic with valid IP origination, this policy should ideally also be implemented at the ISP level (RFC 2827 \parencite{6j}) but it is unclear how widely this is practised. Research should identify whether this is a desirable feature.
    \item Crucible can support unlimited commands, but each command name must be unique, per beacon value, to prevent replay attacks. Further consideration should be made into how multiple command {\it names} can be leveraged to enable multiple executions of the same command, under a single beacon value.
    \item An examination of other cryptocurrencies may provide alternate sources of random beacons, particularly some, such as ethereum, produce blocks more frequently. This research should extend to other sources of publicly verifiable blockchains. Instead of using HTTPS to pull down block values, blockchain networked protocols may provide an alternate source for the random beacons. Further research is required into the feasibility of using malicious block values to influence the beacon, when the result is hashed, at least once, with keys. 
\end{itemize}

% future directions for beacons, for ZKP and for chaos-based crypto


\section{Personal Reflection}
%Add a ???Personal Reflection??? section, and say how well you managed the work, what things did you take from the course, where were the gaps, how would you do it better next time, etc.

The work was founded on a premise of developing a single port knocking prototype, using the ideas from Chapter 3. Discovering vulnerabilities in the first prototype, late into the process, was an unwelcome surprise, meaning that the project had to be restructured into the development of the three protocols seen in Chapter 4. As a consequence, the dissertation is perhaps now more reflective of the real work that took place behind the scenes, perhaps this discovery was in fact a boon, offering me more freedom to explore the {\it process}, rather than simply the end result. For similar projects in the future, I would try to incorporate a more formal process of prototyping, to prepare for such contingencies.\\

From a technical background, I only had limited experience in scripting, mostly in languages {\it other} than Python. The experience I have gained from developing Crucible is very welcome, though if I had been more accustomed to Python ahead of development, I perhaps could have built a working solution i.e. beyond just a prototype. I also didn't want to step out of my comfort zone, so chose not to develop in a newer (and perhaps more exotic) language, such as GoLang.\\

One of the most challenging aspects of the project was performing the literature review on topics such as zero knowledge proofs. Much of the literature on the topic was theoretical cryptography and mathematics, which I am inexperienced in. Of the works that were referenced in this dissertation, countless others were searched through and passed up for being beyond me, or the scope of the project, and it was particularly difficult finding grounded practical examples of zero knowledge proofs of identity.\\

The project has been challenging and rewarding, and I am lucky to have found a topic that I has managed to combine areas of some of my favourite areas of security, making the long hours go unnoticed.

% framing the piece in formal academic structure lends to a lot of repetition, with slight variations...

==> bib_backup.tex <==
@online{chaosimg,
 author  = "Wikimedia",
 title   = "Ikeda map simulation u=0.918 cropped.png",
 publisher = "Wikimedia Commons",
 year    = "2014",
 urlseen = "24-07-28",
 url     = "https://upload.wikimedia.org/wikipedia/commons/2/29/Ikeda_map_simulation_u%3D0.918_cropped.png",
}

@misc{brace_2008, title="{Messages From John}", url={https://web.archive.org/web/20081201165511/http://www.johnmccain.com//Informing/News/NewsReleases/3168f3a2-e59b-433f-94ea-fb1641323507.htm}, journal={JohnMcCain.com - McCain-Palin 2008}, publisher={http://www.johnmccain.com}, author={Brace, Ernest C}, year={2008}, month={5}} 

@inproceedings{1a,
  title="{sKnock: Port-Knocking for Masses}",
  author={Sel, Daniel and Totakura, Sree Harsha and Carle, Georg},
  booktitle="{Reliable Distributed Systems Workshops (SRDSW), 2016 IEEE 35th Symposium on}",
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@INPROCEEDINGS{1b,
author={D. Sel and S. H. Totakura and G. Carle},
booktitle="{2016 IEEE 35th Symposium on Reliable Distributed Systems Workshops (SRDSW)}",
title="{sKnock: Port-Knocking for Masses}",
year={2016},
volume={},
number={},
pages={1-6},
doi={10.1109/SRDSW.2016.11},
ISSN={},
month={9},}

@article{1c,
  title="{Port--Knocking System using Unilateral Authentication Algorithm}",
  author={Tiwari, Reshma},
  publisher="{International Journal of Scientific and Research Publications}",
  year={2013},
  month={9},
  day={9}
}

@INPROCEEDINGS{1d,
author={V. Srivastava and A. K. Keshri and A. D. Roy and V. K. Chaurasiya and R. Gupta},
booktitle="{2011 International Conference on Emerging Trends in Networks and Computer Communications (ETNCC)}",
title="{Advanced port knocking authentication scheme with QRC using AES}",
year={2011},
volume={},
number={},
pages={159-163},
ISSN={},
month={4},}

@INPROCEEDINGS{1e,
author={H. Liu and Z. Wang and Y. Liu},
booktitle="{2012 13th International Conference on Parallel and Distributed Computing, Applications and Technologies}",
title="{Address Knocking: An Undetectable Authentication Based on IPv6 Address}",
year={2012},
volume={},
number={},
pages={85-89},
doi={10.1109/PDCAT.2012.35},
ISSN={2379-5352},
month={12},}

@INPROCEEDINGS{1f,
author={T. Popeea and V. Olteanu and L. Gheorghe and R. Rughiniş},
booktitle="{2011 RoEduNet International Conference 10th Edition: Networking in Education and Research}",
title="{Extension of a port knocking client-server architecture with NTP synchronization}",
year={2011},
volume={},
number={},
pages={1-5},
doi={10.1109/RoEduNet.2011.5993704},
ISSN={2247-5443},
month={6},}

@INPROCEEDINGS{1g,
author={P. Mehran and E. A. Reza and B. Laleh},
booktitle="{2012 IEEE Symposium on Computers Informatics (ISCI)}",
title="{SPKT: Secure Port Knock-Tunneling, an enhanced port security authentication mechanism}",
year={2012},
volume={},
number={},
pages={145-149},
doi={10.1109/ISCI.2012.6222683},
ISSN={},
month={3},}

@article{1h,
  title="{Closed Port Authentication with Port Knocking}",
  author={Lunsford, Phil and Wright, Evan C},
  journal={age},
  booktitle="{Proceedings of the 2005 American Society for Engineering Education Annual Conference & Exposition}",
  volume={10},
  pages={1},
  year={2005}
}

@InProceedings{1i,
author="Manzanares, Antonio Izquierdo
and M{\'a}rquez, Joaqu{\'i}n Torres
and Estevez-Tapiador, Juan M.
and Castro, Julio C{\'e}sar Hern{\'a}ndez",
editor="Gervasi, Osvaldo
and Gavrilova, Marina L.
and Kumar, Vipin
and Lagan{\'a}, Antonio
and Lee, Heow Pueh
and Mun, Youngsong
and Taniar, David
and Tan, Chih Jeng Kenneth",
title="{Attacks on Port Knocking Authentication Mechanism}",
booktitle="{Computational Science and Its Applications -- ICCSA 2005}",
year="2005",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="1292--1300",
isbn="978-3-540-32309-9"
}


@ARTICLE{1j,
author={E. Bou-Harb and M. Debbabi and C. Assi},
journal={IEEE Communications Surveys Tutorials},
title="{Cyber Scanning: A Comprehensive Survey}",
year={2014},
volume={16},
number={3},
pages={1496-1519},
doi={10.1109/SURV.2013.102913.00020},
ISSN={1553-877X},
month={3},}


@Article{1k,
author="Mileva, Aleksandra
and Panajotov, Boris",
title="{Covert channels in TCP/IP protocol stack}",
journal="Central European Journal of Computer Science",
year="2014",
month="6",
day="01",
volume="4",
number="2",
pages="45--66",
issn="2081-9935",
doi="10.2478/s13537-014-0205-6",
url="https://doi.org/10.2478/s13537-014-0205-6"
}

@Article{1l,
author="Wendzel, Steffen
and Keller, J{\"o}rg",
title="Hidden and under control",
journal="annals of telecommunications - annales des t{\'e}l{\'e}communications",
year="2014",
month="8",
day="01",
volume="69",
number="7",
pages="417--430",
issn="1958-9395",
doi="10.1007/s12243-014-0423-x",
url="https://doi.org/10.1007/s12243-014-0423-x"
}

@INPROCEEDINGS{1m,
author={Z. A. Khan and N. Javaid and M. H. Arshad and A. Bibi and B. Qasim},
booktitle="{2012 IEEE 14th International Conference on High Performance Computing and Communication 2012 IEEE 9th International Conference on Embedded Software and Systems}",
title="{Performance Evaluation of Widely Used Portknoking Algorithms}",
year={2012},
volume={},
number={},
pages={903-907},
doi={10.1109/HPCC.2012.129},
ISSN={},
month={6},}

@INPROCEEDINGS{1n,
author={Jiun-Hau Liew and Shirly Lee and Ivy Ong and Hoon-Jae Lee and Hyotaek Lim},
booktitle="{2010 2nd International Conference on Education Technology and Computer}",
title="{One-Time Knocking framework using SPA and IPsec}",
year={2010},
volume={5},
number={},
doi={10.1109/ICETC.2010.5529780},
ISSN={2155-1812},
month={6},}

@INPROCEEDINGS{1o,
author={F. H. Mohd Ali and R. Yunos and M. A. Mohamad Alias},
booktitle="{Proceedings Title: 2012 International Conference on Cyber Security, Cyber Warfare and Digital Forensic (CyberSec)}",
title="{Simple port knocking method: Against TCP replay attack and port scanning}",
year={2012},
volume={},
number={},
pages={247-252},
doi={10.1109/CyberSec.2012.6246118},
ISSN={},
month={6},}

@INPROCEEDINGS{1p,
author={W. Koch and A. Bestavros},
booktitle="{2016 Fourth IEEE Workshop on Hot Topics in Web Systems and Technologies (HotWeb)}",
title="{PROVIDE: Hiding from Automated Network Scans with Proofs of Identity}",
year={2016},
volume={},
number={},
pages={66-71},
doi={10.1109/HotWeb.2016.20},
ISSN={},
month={10},}

@article{1q,
  title="{Network security using hybrid port knocking}",
  author={Al-Bahadili, Hussein and Hadi, Ali H},
  journal={IJCSNS},
  volume={10},
  number={8},
  pages={8},
  year={2010}
}

@INPROCEEDINGS{1r,
author={B. Mahbooba and M. Schukat},
booktitle="{2017 28th Irish Signals and Systems Conference (ISSC)}",
title="{Digital certificate-based port knocking for connected embedded systems}",
year={2017},
volume={},
number={},
pages={1-5},
doi={10.1109/ISSC.2017.7983645},
ISSN={},
month={6},}

@misc{1s,
  title="{Knock: Practical and secure stealthy servers}",
  author={Kirsch, Julian},
  year={2014},
  url={https://gnunet.org/}
}

@Article{1t,
author="Vasserman, Eugene Y.
and Hopper, Nicholas
and Tyra, James",
title="SilentKnock: practical, provably undetectable authentication",
journal="International Journal of Information Security",
year="2009",
month="4",
day="01",
volume="8",
number="2",
pages="121--135",
issn="1615-5270",
doi="10.1007/s10207-008-0070-1",
url="https://doi.org/10.1007/s10207-008-0070-1"
}

@INPROCEEDINGS{1u,
author={M. Khader and A. Hadi and A. Hudaib},
booktitle="{2016 Cybersecurity and Cyberforensics Conference (CCC)}",
title="{Covert Communication Using Port Knocking}",
year={2016},
volume={},
number={},
pages={22-27},
doi={10.1109/CCC.2016.12},
ISSN={},
month={8},}

@INPROCEEDINGS{1v,
author={R. deGraaf and J. Aycock and M. Jacobson},
booktitle="{21st Annual Computer Security Applications Conference (ACSAC'05)}",
title="{Improved port knocking with strong authentication}",
year={2005},
volume={},
number={},
doi={10.1109/CSAC.2005.32},
ISSN={1063-9527},
month={12},}

@article{1w,
  title="{An Object oriented approach for port knocking}",
  booktitle="{International Journal of New Innovations in Engineering and Technology}",
  author={Sudan Jha},
  journal={IJNIET},
  volume={6},
  number={1},
  year={2016}
}

@article{1x,
  title="{Improved kernel-based port-knocking in linux}",
  author={Kirsch, Julian},
  journal={Technical University of Munich},
  year={2014}
}

@article{1y,
  title="{Authenticated Scalable Port-Knocking}",
  author={Sel, Daniel},
  journal={Technical University of Munich},
  year={2016}
}

@article{1z,
  title="{An Analysis of Port Knocking and Single Packet Authorization}",
  author={Jeanquier, Sebastien},
  journal={Royal Holloway, University of London},
  year={2016}
}

@article{1aa,
  title="{COK: Cryptographic one-time knocking}",
  author={Worth, David},
  booktitle="{Black Hat USA (2004)}",
  year={2004}
}

%@book{1ab,
%  title="{Handbook of applied cryptography},
%  author={Katz, Jonathan and Menezes, Alfred J and Van Oorschot, Paul C and Vanstone, Scott A},
%  year={1996},
%  publisher={CRC press}
%}

@book{1ac,
  title="{Silence on the wire: a field guide to passive reconnaissance and indirect attacks}",
  author={Zalewski, Michal},
  year={2005},
  publisher={No Starch Press}
}

@InProceedings{1ad,
author="Mohamed, KamalEldin
and Wijesekera, Duminda
and Costa, Paulo Cesar",
editor="Younas, Muhammad
and Awan, Irfan
and Holubova, Irena",
title="{An Authentication Mechanism for Accessing Mobile Web Services}",
booktitle="{Mobile Web and Intelligent Information Systems}",
year="2017",
publisher="Springer International Publishing",
address="Cham",
pages="147--162",
isbn="978-3-319-65515-4"
}

@article{1ae,
title = "{Towards port-knocking authentication methods for mobile cloud computing}",
journal = "Journal of Network and Computer Applications",
volume = "97",
pages = "66 - 78",
year = "2017",
issn = "1084-8045",
doi = "https://doi.org/10.1016/j.jnca.2017.08.018",
url = "http://www.sciencedirect.com/science/article/pii/S1084804517302813",
author = "Suleman Khan and Muhammad Shiraz and Laleh Boroumand and Abdullah Gani and Muhammad-Khurram Khan",
}

@article{1af,
  title="{Virtualization Technique for port-knocking in mobile cloud computing}",
  author={Boroumand, Laleh and Shiraz, Muhammad and Gani, Abdullah},
  journal={Int. J. Advanced Soft Comput. Appl},
  volume={6},
  number={1},
  year={2014}
}

@inproceedings{1ag,
  title="{BridgeSPA: Improving Tor bridges with single packet authorization}",
  author={Smits, Rob and Jain, Divam and Pidcock, Sarah and Goldberg, Ian and Hengartner, Urs},
  booktitle="{Proceedings of the 10th annual ACM workshop on Privacy in the electronic society}",
  pages={93--102},
  year={2011},
  organization={ACM}
}

@book{1ah,
  title="{Practical cryptography}",
  author={Ferguson, Niels and Schneier, Bruce},
  volume={23},
  year={2003},
  publisher={Wiley New York}
}


%######################################
%######################################

@book{2m,
  title="{Modern cryptography, probabilistic proofs and pseudorandomness}",
  author={Goldreich, Oded},
  volume={17},
  year={1998},
  publisher={Springer Science \& Business Media}
}

@book{2n,
  title="{Encyclopedia of cryptography and security}",
  author={Van Tilborg, Henk CA and Jajodia, Sushil},
  year={2014},
  publisher={Springer Science \& Business Media}
}

@article{2d,
  title="{Zero knowledge proofs: A survey}",
  author={Jain, Gaurav},
  publisher={Citeseer},
  publisher={University of Pennsylvania.}
}

@article{2e,
  title="{A survey of zero-knowledge proofs with applications to cryptography}",
  author={Mohr, Austin},
  url={austinmohr.com}
}

@book{2f,
  title="{Cryptography and Zero Knowledge}",
  author={Mollin, RA},
  year={2006},
  publisher={University of Calgary. Department of Mathematics and Statistics},
  journal={IJPAM},
  volume={31},
  number={3}
}

@article{2g,
  title="{Identification with zero knowledge protocols}",
  author={Giani, Annarita},
  journal={SANS institute Reading room},
  year={2001}
}

@article{2h,
  title="{A survey of zero-knowledge proof for authentication}",
  author={Kurmi, Jitendra and Sodhi, Ankur},
  journal={Int J Adv Res Comput Sci Softw Eng},
  volume={5},
  number={1},
  year={2015}
}

@phdthesis{2i,
  title="{Comparison of Zero Knowledge Authentication Protocols}",
  author={Paramanik, Subhasish},
  publisher={National Institute of Technology, Rourkela},
  year={2014}
}

@article{2j,
  title="{Zero-Knowledge Proof and Authentication Protocols}",
  author={Lipton, Benjamin},
  year={2016},
  url={https://pdfs.semanticscholar.org/abef/6af0025f063d927699eccb6edeedd394dc9a.pdf}
}

@article{2k,
  title="{A primer on zero knowledge protocols}",
  author={Simari, Gerardo I},
  publisher={Universidad Nacional del Sur}
}

%@article{goldwasser1996lecture,
%  title="{Lecture notes on cryptography},
%  author={Goldwasser, Shafi and Bellare, Mihir},
%  publisher={Massachusetts Institute of Technology},
%  year={2008}
%}

@book{2a,
  title="{Applied cryptography: protocols, algorithms, and source code in C}",
  author={Schneier, Bruce},
  year={2007},
  publisher={john wiley \& sons}
}

@book{2b,
  title="{Foundations of cryptography: volume 2, basic applications}",
  author={Goldreich, Oded},
  year={2009},
  publisher={Cambridge university press}
}

@book{2c,
  title="{Modern cryptography: theory and practice}",
  author={Mao, Wenbo},
  year={2003},
  publisher={Prentice Hall PTR}
}

@book{2l,
  title="{Handbook of applied cryptography}",
  author={Katz, Jonathan and Menezes, Alfred J and Van Oorschot, Paul C and Vanstone, Scott A},
  year={1996},
  publisher={CRC press}
}

%######################################
%######################################

@incollection{3a,
title = "{8 - The Rise of the Subversive Multivector Threat}",
editor = "Will Gragido and John Pirc",
booktitle = "{Cybercrime and Espionage}",
publisher = "Syngress",
address = "Boston",
pages = "135 - 151",
year = "2011",
isbn = "978-1-59749-613-1",
doi = "https://doi.org/10.1016/B978-1-59749-613-1.00008-X",
url = "http://www.sciencedirect.com/science/article/pii/B978159749613100008X",
author = "Will Gragido and John Pirc"
}

@article{3b,
  title="{Some basic cryptographic requirements for chaos-based cryptosystems}",
  author={Alvarez, Gonzalo and Li, Shujun},
  journal={International Journal of Bifurcation and Chaos},
  volume={16},
  number={08},
  pages={2129--2151},
  year={2006},
  publisher={World Scientific}
}

@Inbook{3c,
author="Xiao, Di
and Liao, Xiaofeng
and Deng, Shaojiang",
editor="Kocarev, Ljupco
and Lian, Shiguo",
title="{Chaos Based Hash Function}",
bookTitle="{Chaos-Based Cryptography: Theory,Algorithms and Applications}",
year="2011",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="137--203",
isbn="978-3-642-20542-2",
doi="10.1007/978-3-642-20542-2_5",
url="https://doi.org/10.1007/978-3-642-20542-2_5"
}

@ARTICLE{3d,
author={L. Kocarev},
journal="{IEEE Circuits and Systems Magazine}",
title="{Chaos-based cryptography: a brief overview}",
year={2001},
volume={1},
number={3},
pages={6-21},
doi={10.1109/7384.963463},
ISSN={1531-636X},
month={},}

@ARTICLE{3e,
author={C. E. Shannon},
journal="{The Bell System Technical Journal}",
title="{Communication theory of secrecy systems}",
year={1949},
volume={28},
number={4},
pages={656-715},
keywords={},
doi={10.1002/j.1538-7305.1949.tb00928.x},
ISSN={0005-8580},
month={10},}

@INPROCEEDINGS{3f,
author={P. Zhen and G. Zhao and L. Min and X. Li},
booktitle="{2014 Ninth International Conference on P2P, Parallel, Grid, Cloud and Internet Computing}",
title="{A Survey of Chaos-Based Cryptography}",
year={2014},
volume={},
number={},
pages={237-244},
doi={10.1109/3PGCIC.2014.69},
ISSN={},
month={11},}

@Article{3g,
author="Teh, Je Sen
and Samsudin, Azman
and Akhavan, Amir",
title="{Parallel chaotic hash function based on the shuffle-exchange network}",
journal="{Nonlinear Dynamics}",
year="2015",
month="8",
day="01",
volume="81",
number="3",
pages="1067--1079",
issn="1573-269X",
doi="10.1007/s11071-015-2049-6",
url="https://doi.org/10.1007/s11071-015-2049-6"
}

@article{3h,
title = "A fast and efficient chaos-based keyed hash function",
journal = "{Communications in Nonlinear Science and Numerical Simulation}",
volume = "18",
number = "1",
pages = "109 - 123",
year = "2013",
issn = "1007-5704",
doi = "https://doi.org/10.1016/j.cnsns.2012.06.019",
url = "http://www.sciencedirect.com/science/article/pii/S100757041200281X",
author = "A. Kanso and M. Ghebleh",
}

@article{3i,
author = {Chong Fu and Jun-jie Chen and Hao Zou and Wei-hong Meng and Yong-feng Zhan and Ya-wen Yu},
journal = {Opt. Express},
number = {3},
pages = {2363--2378},
publisher = {OSA},
title = "{A chaos-based digital image encryption scheme with an improved diffusion strategy}",
volume = {20},
month = {1},
year = {2012},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-20-3-2363},
doi = {10.1364/OE.20.002363},
}

@article{3j,
  author    = {Jacques M. Bahi and
               Jean{-}Fran{\c{c}}ois Couchot and
               Christophe Guyeux},
  title     = "{Quality Analysis of a Chaotic Proven Keyed Hash Function}",
  journal   = {CoRR},
  volume    = {abs/1608.05928},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.05928},
  archivePrefix = {arXiv},
  eprint    = {1608.05928},
  timestamp = {Wed, 07 Jun 2017 14:40:10 +0200}
}

@INPROCEEDINGS{3k,
author={W. San-Um and W. Srichavengsup},
booktitle="{2013 IEEE International Conference on Communication, Networks and Satellite (COMNETSAT)}",
title="{A topologically simple keyed hash function using a single robust absolute-value chaotic map}",
year={2013},
volume={},
number={},
pages={95-99},
doi={10.1109/COMNETSAT.2013.6870868},
ISSN={},
month={12},}

%######################################
%######################################

@article{4a,
title = "Transaction protection by beacons",
journal = "{Journal of Computer and System Sciences}",
volume = "27",
number = "2",
pages = "256 - 267",
year = "1983",
issn = "0022-0000",
doi = "https://doi.org/10.1016/0022-0000(83)90042-9",
url = "http://www.sciencedirect.com/science/article/pii/0022000083900429",
author = "Michael O. Rabin"
}

@InProceedings{4b,
author="Jiwa, Azad
and Seberry, Jennifer
and Zheng, Yuliang",
editor="Gollmann, Dieter",
title="Beacon based authentication",
booktitle="Computer Security --- ESORICS 94",
year="1994",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="123--141",
isbn="978-3-540-49034-0"
}

@misc{4c,
    author = {Jeremy Clark and Urs Hengartner},
    title = "{On the Use of Financial Data as a Random Beacon}",
    howpublished = "{Cryptology ePrint Archive, Report 2010/361}",
    year = {2010},
    url={https://eprint.iacr.org/2010/361}
}

@InProceedings{4d,
author="Lee, Hui Huang
and Chang, Ee-Chien
and Chan, Mun Choon",
editor="Barni, Mauro
and Herrera-Joancomart{\'i}, Jordi
and Katzenbeisser, Stefan
and P{\'e}rez-Gonz{\'a}lez, Fernando",
title="{Pervasive Random Beacon in the Internet for Covert Coordination}",
booktitle="{Information Hiding}",
year="2005",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="53--61",
isbn="978-3-540-31481-3"
}

@article{4e,
  title="{Trust, and public entropy: a unicorn hunt}",
  author={Lenstra, Arjen K and Wesolowski, Benjamin},
  publisher="{Swiss National Science Foundation}",
  year={2016}
  
}

@misc{4f,
    author = {Joseph Bonneau and Jeremy Clark and Steven Goldfeder},
    title = "{On Bitcoin as a public randomness source}",
    howpublished = "{Cryptology ePrint Archive, Report 2015/1015}",
    year = {2015},
    url={https://eprint.iacr.org/2015/1015}
}

@article{4g,
  author    = {Charles H. Bennett and
               John A. Smolin},
  title     = "{Trust enhancement by multiple random beacons}",
  journal   = "{CoRR}",
  volume    = {cs.CR/0201003},
  year      = {2002},
  url       = {http://arxiv.org/abs/cs.CR/0201003},
  timestamp = {Wed, 07 Jun 2017 14:42:17 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/cs-CR-0201003},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{4h,
    author = "Boneh, Dan and Bonneau, Joseph and Bünz, Benedikt and Fisch, Ben",
    title = "{Verifiable Delay Functions}",
    howpublished = "{Cryptology ePrint Archive, Report 2018/601}",
    year = {2018},
    url={https://eprint.iacr.org/2018/601},
}

@book{4i,
  Author = {Conrad Barski and Chris Wilmer},
  Title = "{Bitcoin for the Befuddled}",
  Publisher = {No Starch Press},
  Year = {2014},
}
@misc{4j, 
    title="{Bitcoin beacon: using the blockchain to generate random bits}", 
    url={http://charlesjlee.com/post/20170716-bitcoin-beacon/}, 
    journal={Charles Lee}, 
    author={Lee, Charles J}, 
    year={2017}, month={7}} 

%######################################
%######################################


@article{5a,
  title="{NIST special publication 800-57}",
  author={Barker, Elaine and Barker, William and Burr, William and Polk, William and Smid, Miles},
  journal="{NIST Special publication}",
  volume={800},
  number={57},
  pages={1--142},
  year={2014}
}

@misc{5b,
    author = {Jos Wetzels},
    title = "{Open Sesame: The Password Hashing Competition and Argon2}",
    howpublished = "{Cryptology ePrint Archive, Report 2016/104}",
    year = {2016},
    url={https://eprint.iacr.org/2016/104}
}

@INPROCEEDINGS{5d,
author={A. Biryukov and D. Dinu and D. Khovratovich},
booktitle="{2016 IEEE European Symposium on Security and Privacy (EuroS P)}",
title="{Argon2: New Generation of Memory-Hard Functions for Password Hashing and Other Applications}",
year={2016},
volume={},
number={},
pages={292-302},
doi={10.1109/EuroSP.2016.31},
ISSN={},
month={3},}

@misc{5g, 
title="{pyblake2 - BLAKE2 hash function for Python}", 
url={https://pythonhosted.org/pyblake2/},
author={Sokolovskiy, Alexandr}, 
year={2013}} 

@misc{5h , 
title="{fast secure hashing}", 
url={https://blake2.net/}, 
journal="{BLAKE2}", 
author={Aumasson, Jean-Philippe and Neves, Samuel and Wilcox-O'Hearn, Zooko and Winnerlein , Christian}} 

%######################################
%######################################


@InProceedings{6a,
author="Bird, Ray
and Gopal, Inder
and Herzberg, Amir
and Janson, Phil
and Kutten, Shay
and Molva, Refik
and Yung, Moti",
editor="Feigenbaum, Joan",
title="Systematic Design of Two-Party Authentication Protocols",
booktitle="{Advances in Cryptology --- CRYPTO '91}",
year="1992",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="44--61",
isbn="978-3-540-46766-3"
}

@article{6c,
  title="{Detection of Promiscuous Nodes Using ARP Packets}",
  author={Sanai, Daiji},
  url={www.securityfriday.com/promiscuous_detection_01.pdf},
  year={2001},
  conference="{Black Hat USA 2001}"
}

@MISC{6d,
  title = {{CVE}-2011-1935},
  howpublished = "Available from MITRE, {CVE-ID} {CVE}-2011-1935.",
  year = {2011},
  url={https://nvd.nist.gov/vuln/detail/CVE-2011-1935},
}

@MISC{6e,
  title = {{CVE}-2014-4174},
  howpublished = "Available from MITRE, {CVE-ID} {CVE}-2014-4174.",
  year = {2014},
  url={https://nvd.nist.gov/vuln/detail/CVE-2014-4174},
}
@article{6f,
  title="{Guide to intrusion detection and prevention systems (idps)}",
  author={Scarfone, Karen and Mell, Peter},
  journal={NIST special publication},
  volume={800},
  number={2007},
  pages={94},
  year={2007}
}

@misc{6g, 
title="{Backdoored Python Library Caught Stealing SSH Credentials}", 
url={https://www.bleepingcomputer.com/news/security/backdoored-python-library-caught-stealing-ssh-credentials/}, 
journal={BleepingComputer}, 
publisher={BleepingComputer.com}, 
author={Cimpanu, Catalin}, 
year={2018}, month={5}} 

@misc{6h,
title="{NCSC advice: Malicious software used to illegally mine cryptocurrency}", 
url={https://www.ncsc.gov.uk/guidance/ncsc-advice-malicious-software-used-illegally-mine-cryptocurrency}, 
journal={NCSC Site}, 
author={NCSC}, 
year={2018}, month={2}} 

@misc{6i, 
title="{Software >> knockknock}", 
url={https://moxie.org/software/knockknock/}, 
journal={Moxie Marlinspike >> Software >> sslstrip}, 
author={Marlinspike, Moxie}} 


@techreport{5c,
  author = {Alex Biryukov and Daniel Dinu and Dmitry Khovratovich and Simon Josefsson},
  title = "{The memory-hard Argon2 password hash and proof-of-work function}",
  howpublished = {Working Draft},
  type = {Internet-Draft},
  number = {draft-irtf-cfrg-argon2-03},
  year = {2017},
  month = {8},
  institution = {IETF Secretariat},
  url = {http://www.ietf.org/internet-drafts/draft-irtf-cfrg-argon2-03.txt},

}

@techreport{5f,
  author = {M-J. Saarinen and J-P. Aumasson},
  title = "{The BLAKE2 Cryptographic Hash and Message Authentication Code (MAC)}",
  howpublished = {Internet Requests for Comments},
  type = {RFC},
  number = {7693},
  year = {2015},
  month = {11},
  issn = {2070-1721},
  publisher = {RFC Editor},
  institution = {RFC Editor},
}

@techreport{6j,
  author = {P. Ferguson and D. Senie},
  title = "{Network Ingress Filtering: Defeating Denial of Service Attacks which employ IP Source Address Spoofing}",
  howpublished = {Internet Requests for Comments},
  type = {BCP},
  number = {38},
  year = {2000},
  month = {5},
  issn = {2070-1721},
  publisher = {RFC Editor},
  institution = {RFC Editor},
  url = {http://www.rfc-editor.org/rfc/rfc2827.txt}}
  
 @book{serious,
  Author = {Jean-Philippe Aumasson},
  Title = "{Serious Cryptography: A Practical Introduction to Modern Encryption}",
  Publisher = {No Starch Press},
  Year = {2017},
  ISBN = {1593278268},
} 
 
